A Complexity Map of Probabilistic Reasoning for Neurosymbolic Classification Techniques

Neurosymbolic artificial intelligence is a growing field of research aiming to combine neural network learning capabilities with the reasoning abilities of symbolic systems. Informed multi-label classification is a sub-field of neurosymbolic AI which studies how to leverage prior knowledge to improve neural classification systems. Recently, a family of neurosymbolic techniques for informed classification based on probabilistic reasoning has gained significant traction. Unfortunately, depending on the language used to represent prior knowledge, solving certain probabilistic reasoning problems can become prohibitively hard when the number of classes increases. Therefore, the asymptotic complexity of probabilistic reasoning is of cardinal importance to assess the scalability of such techniques. In this paper, we develop a unified formalism for four probabilistic reasoning problems. Then, we compile several known and new tractability results into a single complexity map of probabilistic reasoning. We build on top of this complexity map to characterize the domains of scalability of several techniques. We hope this work will help neurosymbolic AI practitioners navigate the scalability landscape of probabilistic neurosymbolic techniques.

==> cardinal.tex <==
Cardinal constraints operate on the number of active variables in a valid state. These constraints can be captured by the \texttt{Cardinal} language, a fragment of \texttt{BLP} where theories consist in a single linear constraint $\langle \mathbf{Y}, \mathbf{1} \rangle \diamond l$ with $\diamond \in \{\leq, \geq, =\}$ and $l \in \mathbb{N}$. Cardinal constraints were first thought as \texttt{PQE}-intractable in \cite{pogancic_differentiation_2019}. However, \cite{AhmedICLR23} developed a polynomial time (and differentiable) algorithm to compute marginal quantities (including \texttt{PQE}) on k-subset constraints (\ie cardinal constraints reduced to $=$). In this section, we show that cardinal constraints can be compiled to \texttt{d-DNNF}, extending known tractability results to all reasoning problems tractable for \texttt{d-DNNF} (including \texttt{ThreshEnum} and \texttt{EQE}). The \texttt{CARD} language defined in \cite{LeBerre2018} is way more expressive than the \texttt{Cardinal} fragment described above as it allows conjunction of cardinal constraints on literals and not only variables. This explains why \texttt{Cardinal} can be compiled to \texttt{d-DNNF} (and even \texttt{OBDD}) while \texttt{CARD} cannot.

Figures \ref{fig:link_nodes} gives a recursive template to compile in polynomial time (create all decision nodes and connect them appropriately) a cardinal constraint $\langle \mathbf{Y}_{1:k}, \mathbf{1} \rangle=l$ into a \textbf{succinct} \texttt{d-DNNF}.

\begin{figure}[htb]
    \hfill
    \begin{subfigure}[t]{0.3\linewidth}
        % \centering
        \includegraphics[width=\textwidth]{circuits/link/Node_1in1.png}
        \caption{$C_1^1$}
        \label{fig:link_C11}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\linewidth}
        % \centering
        \includegraphics[width=\textwidth]{circuits/link/Node_0in1.png}
        \caption{$C_0^1$}
        \label{fig:link_C01}
    \end{subfigure}
    \hfill \break
    % \newline
    
    \begin{subfigure}[t]{0.3\linewidth}
        % \centering
        \includegraphics[width=\textwidth]{circuits/link/Node_0ink.png}
        \caption{$C_0^k$ for $k>1$}
        \label{fig:link_C0k}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\linewidth}
        % \centering
        \includegraphics[width=\textwidth]{circuits/link/Node_link.png}
        \caption{$C_l^k$ for $0<l<k$}
        \label{fig:link_Clk}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\linewidth}
        % \centering
        \includegraphics[width=\textwidth]{circuits/link/Node_kink.png}
        \caption{$C_k^k$ for $k>1$}
        \label{fig:link_Clk}
    \end{subfigure}

\caption{Decision nodes $C_l^k$}
\label{fig:link_nodes}
\end{figure}

\begin{proposition}
    Circuit rooted in $C_l^k$ has size polynomial in $k$.
\end{proposition}

\begin{proof}
    $C_l^k$ contains nodes $(C_i^j)_{1 \leq j \leq k, 0 \leq i \leq \min(j, l)}$ with $6$ wires each, meaning that the size of $C_l^k$ is in $\mathcal{O}(k^2)$.
\end{proof}

\begin{proposition} \label{prop:cardinal_dDNNF}
    For any $k \geq 1$ and $0 \leq l \leq k$ the circuit rooted in $C_l^k$ is a \texttt{d-DNNF}.
\end{proposition}

\begin{proof}
    We can see by recurrence on $k$ that $C_l^k$ contains variables $\{Y_j\}_{1 \leq j \leq k}$. There, we can also show by recurrence on $k$ that $\land$-nodes in $C_l^k$ are \textbf{decomposable}: for the first two $\land$-nodes, the left side contains variable $Y_k$ while the right side contains either no variables or variables $\{Y_j\}_{1 \leq j \leq k-1}$, the remaining $\land$-nodes belonging to sub-circuits $(C_i^j)_{1 \leq j \leq k, 0 \leq i \leq \min(j, l)}$ are decomposable by virtue of the recurrence hypothesis. Again by recurrence on $k$, we can see that $C_l^k$ is \textbf{deterministic}: the root $\lor$-node is deterministic because one side entails $Y_k$ and the other $\neg Y_k$, the remaining $\lor$-nodes belonging to sub-circuits are deterministic by virtue of the recurrence hypothesis.
\end{proof}

\begin{remark}
    It is easy to see that $C_l^k$ is even an \texttt{OBDD} as $\lor$-nodes are decision nodes ordered by the natural order on $\{Y_j\}_{1 \leq j \leq k}$.
\end{remark}
\vspace{5mm}
\begin{proposition}
    The circuit $C_l^k$ with $k \geq 1$ and $0 \leq l \leq k$ accepts a state $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{i:k}}$ iff it contains exactly $l$ variables (ie. $|\mathbf{y}|=l$).
\end{proposition}

\begin{proof}
    Proof by recurrence on $k$ starting at $k=1$:
    \begin{itemize}
        \item Initialization for $k=1$: $C_1^1$ only accepts $y_1=1$ and $C_0^1$ only accepts $y_1=0$.
        \item Heredity from $k$ to $k+1$, for $0 \leq l \leq k$ and $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{i:k+1}}$:
        \begin{itemize}
            \item if $l=0$: $C_0^{k+1}(\mathbf{y})=1$ iff $y_{k+1}=0$ and $C_0^k(\mathbf{y}_{i:k})=1$, which means $C_0^{k+1}$ accepts $\mathbf{y}$ iff:
            $$|\mathbf{y}|=|\mathbf{y}_{i:k}|+y_{k+1}=0+0=0$$
            \item if $l>0$: $C_l^{k+1}(\mathbf{y})=1$ in only two cases:
            \begin{itemize}
                \item if $y_{k+1}=0$ and $C_l^k(\mathbf{y}_{i:k})=1$, which means we have: $$|\mathbf{y}|=|\mathbf{y}_{i:k}|+y_{k+1}=l+0=l$$
                \item if $y_{k+1}=1$ and $C_{l-1}^k(\mathbf{y}_{i:k})=1$, which means we have: $$|\mathbf{y}|=|\mathbf{y}_{i:k}|+y_{k+1}=l-1+1=l$$
            \end{itemize}
        \end{itemize}
    \end{itemize}
\end{proof}

\begin{remark}
    The template on Figure \ref{fig:link_nodes} can be easily modified to compile a cardinal constraint $\langle \mathbf{Y}_{1:k}, \mathbf{1} \rangle \leq l$ into a \textbf{succinct} \texttt{d-DNNF} by replacing $C^1_1$ and $C^k_k$ nodes by $\top$ nodes. Similarly, cardinal constraints $\langle \mathbf{Y}_{1:k}, \mathbf{1} \rangle \geq l$ can be compiled to \texttt{d-DNNF}.
\end{remark}

==> circuits.tex <==
A circuit over variables $\mathbf{Y}$ is a node labeled directed acyclic graph $C=(N, W, \lambda)$ such that:
\begin{itemize}
    \item $N$ is a set of nodes called \textbf{gates}
    \item $W \in N^2$ is a set of edges called \textbf{wires}
    \item $(N, W)$ is directed acyclic graph with a unique sink $g_0 \in N$
    \item $\lambda: N \mapsto \{\land, \lor, \neg, \top, \bot\} \cup \mathbf{Y}$
    \item if $(h, g) \in W$, then gate $h$ is called an \textbf{input} of gate $g$
    \item for all $g \in N$:
    \begin{itemize}
        \item if $\lambda(g) \in \{\top, \bot\}$, then $g$ is a \textbf{constant gate} and has no input
        \item if $\lambda(g) \in \mathbf{Y}$, then $g$ is a \textbf{variable gate} and has no input
        \item if $\lambda(g) = \neg$, then $g$ is a \textbf{negation gate} and has one input
        \item if $\lambda(g) = \land$ (respectively $\lambda(g) = \lor$), then $g$ is a $\land$-gate (respectively $\lor$-gate) must have at least one input
    \end{itemize}
\end{itemize}
The size of a circuit is its number of wires, ie. $|C|:=|W|$.

==> complexitytab.tex <==
% \begin{table}[h]
%     \begin{center}
%     \begin{tabular}{||l|c c c c c||}
%         \hline\hline
%         Classes & Treewidth & Enumerability & SAT & MPE & PQE \\
%         \hline
%         General & $\mathcal{O}(k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ \\
%         \hline
%         2-Horn & $\mathcal{O}(k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ \\
%         \multicolumn{1}{||r|}{Taxonomic} & 1 & $\mathcal{O}(2^k)$ & $\mathcal{O}(1)$ & $\mathcal{O}(k)$ & $\mathcal{O}(k)$ \\
%         \multicolumn{1}{||r|}{Saturated and tree-like HEX} & $\mathcal{O}(k)$ & $\mathcal{O}(k)$ & $\mathcal{O}(1)$ & $\mathcal{O}(k)$ & $\mathcal{O}(k)$ \\
%         Multi-categorical & $\mathcal{O}(k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(1)$ & $\mathcal{O}(k)$ & $\mathcal{O}(k)$ \\
%         Recursive functions & $\tau$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(1)$ & $\mathcal{O}(k2^{\tau})$ & $\mathcal{O}(k2^{\tau})$ \\
%         Exactly l-in-k functions & $\mathcal{O}(k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(1)$ & $\mathcal{O}(k^2)$ & $\mathcal{O}(k^2)$ \\
%         Simple paths in directed graphs & - & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ \\
%         \multicolumn{1}{||r|}{Simple paths in DAG} & $\mathcal{O}(k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(1)$ & $\mathcal{O}(k^3)$ & $\mathcal{O}(k^3)$ \\
%         Matchings & $\mathcal{O}(k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(k^d)$ & $\mathcal{O}(k^d)$ & $\mathcal{O}(2^k)$ \\
%         \hline\hline
%     \end{tabular}
%     \caption{Summary of tractability for common classes (under P $\ne$ NP assumption)}
%     \label{tab:summary}
%     \end{center}
% \end{table}

% \begin{table}[h]
%     \begin{center}
%     \begin{tabular}{||l|c c c c c||}
%         \hline\hline
%         Classes & Bounded treewidth & Enumerability & SAT & MPE & PQE \\
%         \hline
%         General & \xmark & \xmark & \xmark & \xmark & \xmark \\
%         \hline
%         2-Horn & \xmark & \xmark & \xmark & \xmark & \xmark \\
%         \multicolumn{1}{||r|}{Taxonomic} & \cmark & \xmark & \cmark & \cmark & \cmark \\
%         \multicolumn{1}{||r|}{Saturated and tree-like HEX} & \xmark & \cmark & \cmark & \cmark & \cmark \\
%         Multi-categorical & \xmark & \xmark & \cmark & \cmark & \cmark \\
%         % Recursive functions & \cmark & \xmark & \cmark & \cmark & \cmark \\
%         Exactly l-in-k functions & \xmark & \xmark & \cmark & \cmark & \cmark \\
%         Simple paths in directed graphs & - & \xmark & \xmark & \xmark & \xmark \\
%         \multicolumn{1}{||r|}{Simple paths in DAG} & \xmark & \xmark & \cmark & \cmark & \cmark \\
%         Matchings & \xmark & \xmark & \cmark & \cmark & \xmark \\
%         \hline\hline
%     \end{tabular}
%     \caption{Summary of tractability for common classes (under P $\ne$ NP assumption)}
%     \label{tab:summary}
%     \end{center}
% \end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{l c c c c}
        \hline
        \textbf{Languages} & \texttt{MPE} & \texttt{ThreshEnum} & \texttt{PQE} & \texttt{EntQE}\\
        \hline
        \multicolumn{4}{l}{\textbf{Complete}} \\
        \texttt{PL} & \xmark & \xmark & \xmark & \xmark \\
        % \multicolumn{1}{r}{\texttt{Bounded}-$\tau$ \texttt{CNF}} & \cmark & \cmark & \cmark & \cmark \\
        \texttt{BLP} & \xmark & \xmark & \xmark & \xmark \\
        % \multicolumn{1}{r}{\texttt{IntLP}} & \cmark & ? & \xmark \\
        % \texttt{ASP} & \xmark & \xmark & \xmark \\
        \texttt{Circuits} & \xmark & \xmark & \xmark & \xmark \\
        \multicolumn{1}{r}{\texttt{DNNF}} & \cmark & \cmark & \xmark & \xmark \\
        \multicolumn{1}{r}{\texttt{d-DNNF}} & \cmark & \cmark & \cmark & \cmark \\
        \\
        \multicolumn{4}{l}{\textbf{Succinct}} \\
        \texttt{Hex} & \xmark & \xmark & \xmark & \xmark \\
        \multicolumn{1}{r}{\texttt{Hierarchical}} & \cmark & \cmark & \xmark & \xmark \\
        \multicolumn{1}{r}{\texttt{T-H}} & \cmark & \cmark & \cmark & \cmark \\
        \multicolumn{1}{r}{\texttt{TE-H}} & \cmark & \cmark & \cmark & \cmark \\
        % Multi-categorical & \xmark & \xmark & \cmark & \cmark & \cmark \\
        % Recursive functions & \cmark & \xmark & \cmark & \cmark & \cmark \\
        \texttt{Cardinal} & \cmark & \cmark & \cmark & \cmark \\
        \texttt{SPath} & \xmark & \xmark & \xmark & \xmark \\
        \multicolumn{1}{r}{\texttt{ASPath}} & \cmark & \cmark & \cmark & \cmark \\
        \texttt{Match} & \cmark & \cmark & \xmark & \xmark \\
        \hline
    \end{tabular}
    \caption{Summary of tractability results: \cmark (resp. \xmark) indicates that a language $\mathcal{F}$ is tractable (resp. intractable, unless \texttt{P=NP}) for a probabilistic reasoning problem. \texttt{T-H} and \texttt{TE-H} respectively stand for \texttt{Tree-Hierarchical} and \texttt{TreeExclusive-Hierarchical}.}
    \label{tab:summary}
\end{table}

==> paths.tex <==
Simple path constraints can be captured through the edge-based directed graphical language \texttt{SPath} where a state $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}}$ satisfies a theory $(G:=(V, E), \varsigma)$ iff the set of selected edges (ie. $\{e \in E | \varsigma(e) \in \mathbf{y}\}$) forms a total simple path in the directed graph $G$. A simple path (sometimes called a self-avoiding path) is a sequence of adjacent edges such that no vertex is visited twice, it is a total simple path when the first vertex is a source of the graph (a vertex with no incoming edge) and the last vertex is a sink (or a target) of the graph (a vertex with no outgoing edge).
\vspace{5mm}
\begin{example}
    An example of an edge-based directed theory $(G:=(V, E), \varsigma)$ is given on Figure \ref{fig:D}. It has one source $s$ and one sink $t$. The states that satisfy this theory regarding the total simple path semantics are $(Y_1, Y_4)$, $(Y_1, Y_3, Y_5, Y_6)$ and $(Y_2, Y_5, Y_6)$.
\end{example}

\begin{figure}[h]
    \centering
    \begin{tikzpicture}[>=Stealth, node distance=2cm]
      % Nodes
      \node[circle,fill,inner sep=1.5pt, label=above:$s$] (1) {};
      \node[circle,fill,inner sep=1.5pt,right of=1] (2) {};
      \node[circle,fill,inner sep=1.5pt,below of=2] (3) {};
      \node[circle,fill,inner sep=1.5pt,right of=3] (4) {};
      \node[circle,fill,inner sep=1.5pt,right of=2, label=above:$t$] (5) {};
    
      % Edges
      \draw[->] (1) -- node[midway, above] {$Y_1$} (2);
      \draw[->] (1) -- node[midway, left] {$Y_2$} (3);
      \draw[->] (2) -- node[midway, right] {$Y_3$} (3);
      \draw[->] (2) -- node[midway, above] {$Y_4$} (5);
      \draw[->] (3) -- node[midway, below] {$Y_5$} (4);
      \draw[->] (4) -- node[midway, right] {$Y_6$} (5);
    \end{tikzpicture}
    \caption{An edge-based directed theory $(G:=(V, E), \varsigma)$: each edge $e$ is tagged with its corresponding variable $\varsigma(e) \in \mathbf{Y}$.}
    \label{fig:D}
\end{figure}
\vspace{5mm}

Simple path constraints are often encountered informed classification tasks (see Example \ref{ex:WSP1}) or other neurosymbolic AI domains (\eg reinforcement learning on routes \cite{Ling2021}).

\begin{example}[Warcraft Shortest Path] \label{ex:WSP1}
    The Warcraft Shortest Path dataset uses randomly generated images of terrain maps from the Warcraft II tileset. Maps are build on a $12 \times 12$ directed grid (each vertex is connected to all its \textit{neighbors}) and to each vertex of the grid corresponds a tile of the tileset. Each tile is a RGB image that depicts a specific terrain, which has a fixed traveling cost. For each map, the label encodes the shortest s-t path (\ie a path from the upper-left to the lower-right corners), where the weight of the path is the sum of the traveling costs of all terrains (\ie grid vertices) on the path. Terrain costs are used to produce the dataset but are not provided during training nor inference. This dataset has been used several times in the literature to build informed classification tasks to evaluate neurosymbolic techniques \cite{pogancic_differentiation_2019,Yang2020,niepert_implicit_2021,Ahmed2022spl}: prior knowledge about the task tells us that valid labels must correspond to simple paths in the grid.
\end{example}

Probabilistic reasoning as well as knowledge compilation of simple path constraints in undirected graph is a well studied topic \cite{Nishino2017,Choi2017,Shen2019}. In this section we analyze the complexity of probabilistic reasoning for simple path constraints in directed graphs. In particular, we show that the acyclicity of the graph plays a crucial role in the tractability of probabilistic reasoning.

% Simple path boolean functions can be expressed in ASP logic with programs composed of the rules:
% \begin{gather}
%     r_{(s, u)} : Y_{(s, u)} \leftarrow (\text{\textit{not} } Y_{(s, v)})_{\substack{(s, v) \in E \\ v \ne u}} \text{ \textit{for} } (s, u) \in E \\
%     r_{(v, w)} : Y_{(v, w)} \leftarrow (Y_{(u, v)})_{(u, v) \in E}  \text{ \textit{for} } v \in V \setminus s, (v, w) \in E
% \end{gather}
\vspace{5mm}
\begin{proposition}
    \texttt{SPath} is \texttt{MPE}, \texttt{ThreshEnum}, \texttt{PQE} and \texttt{EQE}-intractable.
\end{proposition}

\begin{proof}
    Solving \texttt{MPE} for a \texttt{SPath} theory $(G, \varsigma)$ is equivalent to finding a shortest path in $G$ with (positive and negative) real weights on the edges, which is known to be NP-hard by a polynomial reduction from the Hamiltonian path problem \cite{Karp1972}. This also implies that \texttt{SPath} is \texttt{ThreshEnum}-intractable. Likewise, counting the number of simple paths of a graph $G$ is known to be \#P-hard \cite{valiant1979} and has a trivial polynomial reduction to solving \texttt{PQE} and \texttt{EQE} for a \texttt{SPath} theory $(G, \varsigma)$.
\end{proof}

% A \texttt{SPath} theory $(D, \varsigma)$ is said \textbf{acyclic} if $D$ is a Directed Acyclic Graph (DAG). 

The fragment of \texttt{SPath} composed only of acyclic theories is called \texttt{ASPath}. We note $\mathbf{Y}:=\{Y_i\}_{1 \leq i \leq |E|}$ the set of variables and assume without loss of generality than $\varsigma: E \rightarrow \mathbf{Y}$ is a topological ordering of the edges: for any path, the order of edges in the path is a sub-order of the topological order. For instance, $\varsigma$ in the theory on Figure \ref{fig:D} is a topological ordering of the edges. For simplicity, we note $e_i$ the edge such that $\varsigma(e_i)=Y_i$. For a vertex $u \in V$, we will note $\varsigma_m(u)$ the index of the first incident edge to $u$ and $\varsigma_M(u)$ the index of the last outgoing edge of $u$. We also note $D^j$ the graph that contains edges $(e_i)_{1 \leq i \leq j}$ and all vertices that are endpoints of those edges. Finally, we can assume without loss of generality that $D$ only contains a single source and sink. If not: chose one source vertex $s$, delete all the others and reconnect their outgoing edges to $s$, and do the same with a sink vertex $t$. This operation can be done in polynomial type and does not change the semantic of the theory (\ie accepted states are left unchanged).

Figure \ref{fig:spk_nodes} and \ref{fig:spi_nodes} represent recursive templates that allow us to compile in polynomial time (create all decision nodes and connect them appropriately) an acyclic and topological simple path theory $(D:=(V, E), \varsigma)$ into a \textbf{succinct} \texttt{d-DNNF} rooted in node $C_t^k$.
\vspace{5mm}
\begin{figure}[b]
\begin{subfigure}[t]{0.30\linewidth}
    \centering
    \includegraphics[width=\textwidth]{circuits/paths/FinalIncomingNode.png}
    \caption{{\scriptsize $C_v^1$ if $e_1=(s, v)$}}
    \label{fig:Cnk_outgoing}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.30\linewidth}
    \centering
    \includegraphics[width=\textwidth]{circuits/paths/FinalNode.png}
    \caption{{\scriptsize $C_v^1$ if $v \neq s$ and $e_1 \neq (s, v)$}}
    \label{fig:Cnk}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.30\linewidth}
    \centering
    \includegraphics[width=\textwidth]{circuits/paths/FinalSourceNode.png}
    \caption{{\scriptsize $C_s^1$}}
    \label{fig:Cs1}
\end{subfigure}
\caption{Initial decision nodes $C_v^1$ for $v \in V$}
\label{fig:spk_nodes}
\end{figure}

\begin{figure}[t]
\hspace*{\fill}
\begin{subfigure}[t]{0.30\linewidth}
    \centering
    \includegraphics[width=\textwidth]{circuits/paths/IncomingNode.png}
    \caption{{\scriptsize $C_v^{i+1}$ if $e_{i+1}=(u, v)$}}
    \label{fig:Cni_outcoming}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.30\linewidth}
    \centering
    \includegraphics[width=\textwidth]{circuits/paths/NotIncomingNode.png}
    \caption{{\scriptsize $C_v^{i+1}$ if $e_{i+1}$ is not an incoming edge of $v$}}
    \label{fig:Cni_not_outcoming}
\end{subfigure}
\hspace*{\fill}
\caption{Decision nodes $C_v^i$ for $1 < i \leq k$ and $v \in V$}
\label{fig:spi_nodes}
\end{figure}

\begin{proposition}
    Circuit $C_t^k$ has size polynomial in the number of edges in $k$.
\end{proposition}

\begin{proof}
    Circuit $C_t^k$ has at most $|V| \times k = \mathcal{O}(k^3)$ decision nodes with $6$ wires each, meaning that the size of the circuit is in $\mathcal{O}(k^3)$.
\end{proof}

\begin{remark}
    Notice that every node $C_v^i$ such that such that $i > \sigma_M(v)$ will not appear in the circuit rooted in $C_t^k$. Similarly, every node $C_v^i$ such that $i < \sigma_m(v)$ is equivalent to $\bot$ and can thus be trimmed of the circuit. Therefore, the size of the trimmed circuit is much smaller that $2k^3$.
\end{remark}
\vspace{5mm}
\begin{proposition}
    For each vertex $v$ and edge $e_i$, the circuit rooted in $C_v^i$ is a \texttt{d-DNNF}.
\end{proposition}

\begin{proof}
    Similar to the proof of Proposition \ref{prop:cardinal_dDNNF}. We can see by recurrence on $i$ that $C_v^i$ contains variables $\{Y_j\}_{1 \leq j \leq i}$. There, we can also show by recurrence on $i$ that $\land$-nodes in $C_v^i$ are \textbf{decomposable}: for the first two $\land$-nodes, the left side contains variable $Y_i$ while the right side contains either no variables or variables $\{Y_j\}_{1 \leq j \leq i-1}$, the remaining $\land$-nodes are decomposable by virtue of the recurrence hypothesis. Again by recurrence on $i$, we can see that $C_v^i$ is \textbf{deterministic}: the root $\lor$-node is deterministic because one side entails $Y_i$ and the other $\neg Y_i$, the remaining $\lor$-nodes belonging to sub-circuits are deterministic by virtue of the recurrence hypothesis.
\end{proof}

\begin{remark}
    It is easy to see that $C_v^i$ is even an \texttt{OBDD} as every $\lor$-nodes are decision nodes ordered by the topological order of the edges.
\end{remark}
\vspace{5mm}
\begin{lemma} \label{lem:topo}
    Assume that edges follow a topological order. If for $i>1$ $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{1:i}}$ represents a total simple path $s \to v$ in $D^i$ and $y_i=1$, then $e_i=(u, v)$ for some $u \in D^{i-1}$.
\end{lemma}

\begin{proof}
    We note $e_i=(u, w)$. We first show that $u \in D^{i-1}$:
    \begin{itemize}
        \item if $u=s$, then $u \in D^1 \subset D^{i-1}$.
        \item if $u \ne s$, since $\mathbf{y}$ represents a path $s \to v$, there is an edge $e_j=(r, u)$ with $j < i$, which means that $u \in D^{i-1}$. 
    \end{itemize}
    
    Now let's show that $w=v$ reasoning by the absurd. Let's assume that $w \ne v$, then since $\mathbf{y}$ represents a path $s \to v$, there is an edge $e_l=(q, v)$ with $l<i$. Hence, there is a path from the end point $w$ of $e_i$ to the start point $q$ of $e_l$ with $l<i$, which is in contradiction with edges following a topological order.

    Therefore we can conclude that $e_i=(u, v)$ for some $u \in D^{i-1}$.
\end{proof}

\begin{lemma} \label{lem:Csi}
    The circuit $C_s^i$ with $1 \leq i \leq k$ only accepts the null state $\mathbf{0} \in \mathbb{B}^{\mathbf{Y}_{1:i}}$.
\end{lemma}

\begin{proof}
    Proof by recurrence on $i$:
    \begin{itemize}
        \item Initialization for $i=1$: $C_s^{1}(y_1)=1$ iff $y_1=0$ by definition (see Figure \ref{fig:Cs1}).
        \item Heredity from $i$ to $i+1$: $s$ has no incoming edge in $D$ (because it is a source vertex), hence $C_s^{i+1}$ accepts $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{1:i+1}}$ iff $y_{i+1}=0$ and $C_s^{i}(\mathbf{y}_{1:i})=1$. Which means by the recurrence hypothesis that $\mathbf{y}_{1:i}=\mathbf{0}$ and therefore $\mathbf{y}=0$.
    \end{itemize}
\end{proof}

\begin{proposition}
    The circuit $C_v^i$ with $1 \leq i \leq k$ and $v \in D^i \setminus s$ accepts a state $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{1:i}}$ iff it is a total simple path in $D^i$. In particular $C_t^k$ is equivalent to $(D, \varsigma)$.
\end{proposition}

\begin{proof}
    We will proceed by recurrence on $i$, first showing that all accepted states by $C_v^i$ are paths $s \to v$ in $D^i$ then showing that only them are accepted.
    \begin{itemize}
        \item Initialization for $i=1$: $D^1$ only contains the vertices $s$ and $v$ such that $e_1=(s, v)$ and $C_v^1$ accepts exactly $y_1=1$ which is the only path $s \to v$ in $D^1$.
        \item Heredity from $i$ to $i+1$:
        \begin{itemize}
            \item Assume a state $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{1:i+1}}$ represents a path $s \to v$ in $D^{i+1}$ and note:
            \begin{itemize}
                \item if $y_{i+1}=1$, then according to Lemma \ref{lem:topo} $e_{i+1}=(u, v)$ for some $u \in D^i$
                \begin{itemize}
                    \item if $u=s$: then $\mathbf{y}_{1:i}=\mathbf{0}$ and by Lemma \ref{lem:Csi} $C_v^{i+1}(\mathbf{y})=C_s^{i}(\mathbf{y}_{1:i})=1$
                    \item if $u \ne s$: then $\mathbf{y}_{1:i}$ represents a path $s \to u$ in $D^i$ and by the recurrence hypothesis $C_v^{i+1}(\mathbf{y})=C_u^i(\mathbf{y}_{1:i})=1$
                \end{itemize}
                \item if $y_{i+1}=0$, then $\mathbf{y}_{1:i}$ represents a path $s \to v$ in $D^i$ and by the recurrence hypothesis $C_v^{i+1}(\mathbf{y})=C_v^i(\mathbf{y}_{1:i})=1$.
            \end{itemize}
            \item Assume a state $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{1:i+1}}$ is accepted by $C_v^{i+1}$:
            \begin{itemize}
                \item if $y_{i+1}=1$, then according to Lemma \ref{lem:topo} $e_{i+1}=(u, v)$ for some $u \in D^i$
                \begin{itemize}
                    \item if $u=s$: then $C_s^{i}(\mathbf{y}_{1:i})=C_v^{i+1}(\mathbf{y})=1$, hence by Lemma \ref{lem:Csi} $\mathbf{y}_{1:i}=\mathbf{0}$ and $\mathbf{y}$ represents a path $s \to v$ in $D^{i+1}$.
                    \item if $u \ne s$: then $C_u^i(\mathbf{y}_{1:i})=C_v^{i+1}(\mathbf{y})=1$, hence by the recurrence hypothesis $\mathbf{y}_{1:i}$ represents a path $s \to u$ in $D^i$ and by adding $e_{i+1}$ $\mathbf{y}$ represents a path $s \to v$ in $D^{i+1}$.
                \end{itemize}
                \item if $y_{i+1}=0$, then $C_u^i(\mathbf{y}_{1:i})=C_u^{i+1}(\mathbf{y})=1$, hence by the recurrence hypothesis $\mathbf{y}_{1:i}$ represents a path $s \to v$ in $D^i$ and by not adding edge $e_{i+1}$ $\mathbf{y}$ represents a path $s \to v$ in $D^{i+1}$.
            \end{itemize}
        \end{itemize}
    \end{itemize}
\end{proof}

Finally, we can state our main result:
\vspace{5mm}
\begin{proposition}
    \texttt{ASPath} is \texttt{MPE}, \texttt{ThreshEnum}, \texttt{PQE} and \texttt{EQE}-tractable.
\end{proposition}

\begin{proof}
    First, it is succinct because it is an edge-based logic. Let's assume an acyclic simple path theory $(G, \varsigma)$. If needed, merge source vertices and sink vertices like mentioned above. Since a topological order of the edges in a DAG can be compiled in a polynomial time, we can compute $\varrho$ such that $(G, \varrho)$ is acyclic and topological. We compile $(G, \varrho)$ into a succinct \texttt{d-DNNF} $C_t^k$ as seen above. We rewrite leaf nodes $Y_i$ to $Y_{\varsigma \circ \varrho^{-1}(i)}$ in the \texttt{d-DNNF}. The new circuit is still a succinct \texttt{d-DNNF} and is equivalent to the theory $(G, \varsigma)$. Finally, by inheritance from \texttt{d-DNNF}, \texttt{ASPath} is \texttt{MPE}, \texttt{ThreshEnum}, \texttt{PQE} and \texttt{EQE}-tractable.
\end{proof}

\begin{example}
    This case gives a great example how a better understanding of knowledge representation and probabilistic reasoning can influence the design of informed classification tasks. In its original version \cite{pogancic_differentiation_2019}, output variables correspond to vertices in the grid and a state satisfies the simple path constraint if the vertices set to $1$ constitute a simple s-t path. As pointed out in \cite{Ahmed2022spl}, the set of vertices ambiguously encode more than one path (because of cycles in the grid, there are several possible simple paths that go through the same vertices). Therefore, \cite{Ahmed2022spl} designs another version of the task where edges of the grid are chosen as output variables instead of vertices. However, because \texttt{SPath} is \texttt{MPE} and \texttt{PQE}-intractable, \cite{Ahmed2022spl} transforms prior knowledge to only keep simple paths with a maximal length of $29$ (the maximal length found in the training set) as valid states. This makes computations tractable but implies that test samples set might not be consistent with prior knowledge (it might contain a path longer than $29$ edges). Finally, such method would not scale to larger grids.
\end{example}

% Let's first give to quick lemmas about circuit $C_s^1$:
% \begin{enumerate}
%     \item a node $C_{v_p}^i$ does not accept a state $\mathbf{y} \in \mathbb{B}^{\mathbf{E}}$ if there is $j>i$ such that all nodes $C_{v_q}^j$ where $v_q$ does not precede $v_p$ in the order (ie. $q \geq p$) does not accept $\mathbf{y}$:
%     \begin{equation}
%         \forall 1\leq i < k, 1 \leq p < m, (\exists j>i, \forall q \geq p, C_{v_q}^j(\mathbf{y}_{j:k})=0) \implies C_{v_p}^i(\mathbf{y}_{i:k})=0
%     \end{equation}
%     \item a node $C_{v_p}^i$ does not accept a state $\mathbf{y} \in \mathbb{B}^{\mathbf{E}}$ if there is a later vertice $v_q$ (ie. $q>p$) such that for all edges $e_j$ the node $C_{v_q}^j$ does not accept $\mathbf{y}$:
%     \begin{equation}
%         \forall 1\leq i < k, 1 \leq p < m, (\exists q>p, \forall 1\leq j  k, C_{v_q}^j(\mathbf{y}_{j:k})=0) \implies C_{v_p}^i(\mathbf{y}_{i:k})=0
%     \end{equation}
% \end{enumerate}

% \begin{lemma} \label{lem:non_terminal}
%     A non-terminal node $C_{v_p}^i$ (ie. where $i<k$) can only accept a state if one of the following nodes $(C_{v_q}^{i+1})_{p \leq q \leq m}$ accepts it.
% \end{lemma}

% \begin{lemma} \label{lem:disconnect}
%     If there is a edge $e_j$ and a vertice $v_p$ such that for all vertices $v_q$ after $v_p$ (ie. $p \leq q$) the node $C_{v_q}^j$ rejects a state $\mathbf{y}$, then for any previous edge $e_i$ (ie. $i \leq j$) and for all vertices $v_q$ after $v_p$ the node $C_{v_q}^i$ also rejects $\mathbf{y}$:
%     \begin{gather} \label{eq:disconnect}
%         \forall 1 \leq j \leq k, 1 \leq p \leq m, \forall \mathbf{y} \in \mathbb{B}^{\mathbf{E}} \notag \\
%         (\forall p \leq q \leq m, C_{v_q}^j(\mathbf{y}_{j:k})=0) \implies (\forall 1 \leq i \leq j, \forall p \leq q \leq m, C_{v_q}^i(\mathbf{y}_{i:k})=0)
%     \end{gather}
% \end{lemma}

% \begin{proof}
%     Assume $1 < j \leq k, 1 \leq p \leq m$ and $\mathbf{y} \in \mathbb{B}^{\mathbf{E}}$ such that:
%     \begin{equation*}
%         \forall p \leq q \leq m, C_{v_q}^j(\mathbf{y}_{j:k})=0
%     \end{equation*}
    
% Let's show by recurrence on $i$ starting at $i=j$ and ending at $i=1$, that:
%     \begin{equation}
%         \forall 1 \leq i \leq j, \forall p \leq q \leq m, C_{v_q}^i(\mathbf{y}_{i:k})=0
%     \end{equation}
%     \begin{itemize}
%         \item Initialization at $i=j$: direct from the hypothesis.
%         \item Heredity from $i+1 \leq j$ to $i$: all nodes in $(C_{v_q}^{i+1})_{p \leq q \leq m}$ reject $\mathbf{y}$, hence applying Lemma \ref{lem:non_terminal} on any node in $(C_{v_q}^{i})_{p \leq q \leq m}$ gives you: $\forall p \leq q \leq m, C_{v_q}^i(\mathbf{y}_{i:k})=0$.
%     \end{itemize}
% \end{proof}

% \begin{lemma} \label{lem:2out}
%     If there is is a vertice $v_d$ with two outcoming edges $e_i$ and $e_j$ ($i<j$) in a state $\mathbf{y}$, then $C_s^1(\mathbf{y})$ rejects $\mathbf{y}$.
% \end{lemma}

% \begin{proof}
%     Assume that there is a vertice $v_d$ with two outcoming edges $e_i=(v_d, v_p)$ and $e_j$ ($i<j$) in $\mathbf{y}$. Let's first show that $C_{v_p}^{i+1}(\mathbf{y}_{i+1:k})=0$:
%     \begin{itemize}
%         \item If $j=i+1$, then because $y_j=1$ and $e_j$ is not an outcoming edge of $v_p$: $C_{v_p}^{i+1}(\mathbf{y}_{i+1:k})=0$.
%         \item If $j > i+1$, then for all $p \leq q \leq m$: $e_j$ is not an outcoming edge of $v_q$, which implies $C_{v_q}^j(\mathbf{y}_{j:k})=0$ since $y_j=1$. Following Lemma \ref{lem:disconnect}, this leads to: $$\forall 1 \leq l \leq j, \forall p \leq q \leq m, C_{v_q}^l(\mathbf{y}_{l:k})=0$$ and in particular to $C_{v_p}^{i+1}(\mathbf{y}_{i+1:k})=0$.
%         % \begin{equation*}
%         %     \forall 1 \leq i \leq j, \forall p \leq q \leq m, C_{v_q}^i(\mathbf{y}_{i:k})=0
%         % \end{equation*}
%     \end{itemize}

%     Since $y_i=1$, $e_i=(v_d, v_p)$ and $C_{v_p}^{i+1}(\mathbf{y}_{i+1:k})=0$, we have: $C_{v_d}^i(\mathbf{y}_{i:k})=0$. Besides, because $y_i=1$ and $e_i$ is not an outcoming edge for all other vertices than $v_d$, then: $$\forall 1 \leq q \ne d \leq m, C_{v_q}^i(\mathbf{y}_{i:k})=0$$

%     Combining both gives:
%     \begin{equation*}
%         \forall 1 \leq q \leq m, C_{v_q}^i(\mathbf{y}_{i:k})=0
%     \end{equation*}

%     Applying Lemma \ref{lem:disconnect} we get:
%     \begin{equation*}
%         \forall 1 \leq l \leq i, \forall 1 \leq q \leq m, C_{v_q}^l(\mathbf{y}_{l:k})=0
%     \end{equation*}

%     In particular with $l=q=1$ this gives: $C_s^1(\mathbf{y})=C_{v_1}^1(\mathbf{y})=0$.
% \end{proof}

% \begin{lemma} \label{lem:1in1out}
%     If there is a non-sink vertice $v_d$ (ie. $d<m$) with an incoming edges $e_i$ and no outcoming edges in a state $\mathbf{y}$, then $C_s^1(\mathbf{y})$ rejects $\mathbf{y}$.
% \end{lemma}

% \begin{proof}
%     Assume that $v_d$ is the first vertice with an incoming edges $e_i$ and no outcoming edges in a state $\mathbf{y}$.
    
%     Let's first show by recurrence on $j$ from $j=k$ to $j=i$ that: $$\forall i \leq j \leq k, C_{v_d}^i(\mathbf{y}_{i:k})=0$$
%     \begin{itemize}
%         \item Initialization $j=k$:
%         \begin{itemize}
%             \item if $e_k=(v_d, t)$, then $y_k=0$ from the hypothesis and $C_{v_d}^k(y_k)=0$
%             \item if $e_k \ne (v_d, t)$, then $C_{v_d}^k(y_k)=0$ by default
%         \end{itemize}
%         \item Heredity from $j+1$ to $j$:
%         \begin{itemize}
%             \item if $e_j=(v_d, v_p)$, then $y_j=0$ from the hypothesis and: $$C_{v_d}^j(\mathbf{y}_{j:k})=C_{v_d}^{j+1}(\mathbf{y}_{j+1:k})=0$$
%             \item if $e_j$ in not an outcoming edge of $v_d$:
%             \begin{itemize}
%                 \item if $y_j=0$: $C_{v_d}^j(\mathbf{y}_{j:k})=C_{v_d}^{j+1}(\mathbf{y}_{j+1:k})=0$
%                 \item if $y_j=1$: $C_{v_d}^j(\mathbf{y}_{j:k})=0$ by default
%             \end{itemize}
%         \end{itemize}
%     \end{itemize}

% \end{proof}


% \begin{enumerate}
%     \item assume there is no outcoming edge of $s$ in $\mathbf{y}$: then by recurrence on nodes $C_s^i$ from $k$ to $1$ $C_s^1(\mathbf{y})=0$.
%     \item assume that there is a node $v_p$ with two outcoming edges $e_i=(v_p, v_q)$ and $e_j$ ($i<j$) in $\mathbf{y}$. Let's  : then $\forall d \geq q, C_{v_d}^j(\mathbf{y}_{j:k})=0$ (because $y_j=1$ and $e_j$ is not an outcoming edge of $v_d$). Follwing Equation \ref{eq:disconnect} this implies that $C_{v_q}^i(\mathbf{y}_{i:k})=0$. Since $y_i=1$, this also implies  and $e_i$ is not an outcoming edge for all other vertices, then $\forall 1 \leq q \leq m$, $C_{v_q}^i(\mathbf{y}_{i:k})=0$, which again from Equation \ref{eq:disconnect} implies $C_s^1(\mathbf{y})=0$.
%     \item assume that there is a node $v_p$ with an incoming edge but no outcoming edge in $\mathbf{y}$:
% \end{enumerate}

% First, assume there is no outcoming edge of $s$ in $\mathbf{y}$: then by recursion on nodes $C_s^i$ from $k$ to $1$ $C_s^1$ evaluates to $\bot$ which is contradictory. Thus there is an outcoming edge of $s$ in $\mathbf{y}$.
% Then assume that there is a node $n$ with two outcoming edges in $\mathbf{y}$.
% Then assume that there is a node $n$ with an incoming edge but no outcoming edge in $\mathbf{y}$.

==> recursive.tex <==
A theory $\kappa \in \mathcal{T}(\mathbf{Y})$ enforces a functional dependency from variables $\mathbf{W} \subset \mathbf{Y}$ onto variables $\mathbf{Z} \subset \mathbf{Y}$, noted , iff any two accepting states that are identical on $\mathbf{W}$ are also identical on $\mathbf{Z}$. A class of theories $(\kappa_k)_{k \in \mathbb{N}^*}$ is (d, m, n)-\textbf{recursive} with $d, m, n \in \mathbb{N}^*$ iff:
    \begin{gather}
        \forall k \leq 1, T_k \in \mathcal{T}(\mathbf{S}_k^{m, n, d}), \\
        \mathbf{A}_{1,:} \to \mathbf{N}_{1,:} \cup \mathbf{M}_{1,:} \\
        \forall k > 1, \forall 1 < j \leq k, \mathbf{A}_{j,:} \cup \mathbf{M}_{j-1,:} \to \mathbf{N}_{j,:} \cup \mathbf{M}_{j,:}
    \end{gather}
where $\mathbf{S}_k^{d, m, n} := \mathbf{A}_{1:k,1:d} \cup \mathbf{M}_{1:k,1:m} \cup \mathbf{N}_{1:k,1:n}$.

\begin{proposition}
    A (m, n, d)-\textbf{recursive} class of theories is tractable.
\end{proposition}

\begin{proof}
    We show here that an (d, m, n)-\textbf{recursive} class of theories can be compiled in polynomial time into a concise class of propositional formulas in conjunctive normal form of bounded treewidth $d + 2m + n$.
\end{proof}

\begin{figure}[h]
    \centering
    \begin{tikzpicture}
      % Draw the first number
      \node (A1) at (0,0) {$\mathbf{A}_{1,:}$};
      \node (A2) at (-2,0) {$\mathbf{A}_{2,:}$};
      \node (A3) at (-4,0) {$\mathbf{A}_{3,:}$};
      \node (Ak) at (-8,0) {$\mathbf{A}_{k,:}$};
      
      % Draw the result under the second number
      \node (N1) at (0, -1) {$\mathbf{N}_{1,:}$};
      \node (N2) at (-2, -1) {$\mathbf{N}_{2,:}$};
      \node (N3) at (-4,-1) {$\mathbf{N}_{3,:}$};
      \node (Nk) at (-8,-1) {$\mathbf{N}_{k,:}$};
      
      % Draw the carry
      \node (M0) at (0, 0.5) {};
      \node (M1) at (-1.25, 0.5) {$\mathbf{M}_{1,:}$};
      \node (M2) at (-3.25, 0.5) {$\mathbf{M}_{2,:}$};
      \node (M3) at (-5.25, 0.5) {$\mathbf{M}_{3,:}$};
      \node (Ck-1) at (-7.25, 0.5) {$\mathbf{M}_{k-1,:}$};
      \node (Mk) at (-9.25, 0.5) {$\mathbf{M}_{k,:}$};

      % Draw cluster names
      \node[color=darkblue] (C1) at (-0.25,1.6) {$\mathbf{C}_1$};
      \node[color=darkpurple] (C2) at (-2.25,1.6) {$\mathbf{C}_2$};
      \node[color=darkbrown] (C3) at (-4.25,1.6) {$\mathbf{C}_3$};
      \node[color=dark] (Ck) at (-8.25,1.6) {$\mathbf{C}_k$};

      % Draw the edges
      \draw (M1) -- (A1);
      \draw (M1) -- (N1);
      \draw (N1) -- (A1);
      \draw (M1) -- (A2);
      \draw (M1) -- (M2);
      \draw (M1) -- (N2);
      \draw (M2) -- (A2);
      \draw (M2) -- (N2);
      \draw (A2) -- (N2);
      \draw (M2) -- (A3);
      \draw (M2) -- (M3);
      \draw (M2) -- (N3);
      \draw (M3) -- (A3);
      \draw (M3) -- (N3);
      \draw (A3) -- (N3);
      \draw (M3) -- (-5.5,-0.25);
      \draw (Ck-1) -- (-6,-0.25);
      \draw (Ck-1) -- (Ak);
      \draw (Ck-1) -- (Mk);
      \draw (Ck-1) -- (Nk);
      \draw (Mk) -- (Nk);
      \draw (Mk) -- (Ak);
      \draw (Mk) -- (Nk);
      \draw (Ak) -- (Nk);
      
      % Draw the cliques
      \draw[edge,color=darkblue,line width=50pt] (M1) -- (M0) -- (A1) -- (N1);
      \draw[edge,color=darkpurple,line width=50pt] (M2) -- (M1) -- (A2) -- (N2) -- (A2);
      \draw[edge,color=darkbrown,line width=50pt] (M3) -- (M2) -- (A3) -- (N3) -- (A3);
      \draw[edge,color=dark,line width=50pt] (Mk) -- (Ck-1) -- (Ak) -- (Nk) -- (Ak);
      % \draw[edge,color=dark,line width=50pt] (Ck-1) -- (-5.75,-0.5);
    
      % Draw dots
      \fill (-5.5,-0.5) circle [radius=1pt];
      \fill (-5.75,-0.5) circle [radius=1pt];
      \fill (-6,-0.5) circle [radius=1pt];
    \end{tikzpicture}
    \caption{Compressed representation of the primal graph of $\kappa_k$. Each node $\mathbf{Y}_{i,:}$ represents a set of variables that forms a clique in the primal graph. An edge between two nodes means that the union of the two sets forms a clique in the primal graph. Highlighted clusters $\mathbf{C}_i$ indicate maxcliques of the primal graph. Notice that clusters naturally arrange in a chain pattern: each one shares variables $\mathbf{M}_{i-1,:}$ with its predecessor and variables $\mathbf{M}_{i,:}$ with its successor. This observation implies that the clusters can be used to build a junction tree of maxcliques of the primal graph.}
    \label{fig:cliques_recursive}
\end{figure}

A sequence of functions $(f_k)_{k \in \mathbb{N}^*}$ is \textbf{recursive} iff:
    \begin{gather}
        \exists m, n, d \in \mathbb{N}^*, \mathcal{I} \subset \mathbb{B}^d, \mathcal{M} \subset \mathbb{B}^m, \mathcal{N} \subset \mathbb{B}^n \notag \\
        \forall k, f_k : \mathcal{I}^k \mapsto \mathcal{M} \times \mathcal{N}^k \\
        \exists g: \mathcal{I} \times \mathcal{M} \mapsto \mathcal{M} \times \mathcal{N} \notag \\
        % \exists \mathbf{o} \in \mathbb{B}^m \notag \\
        \forall k>1, \forall \mathbf{a} \in \mathcal{I}^k, \notag \\
        f_k(\mathbf{a}_{1:k}) = \langle g(\mathbf{a}_k, f_{k-1}(\mathbf{a}_{1:k-1})_{1:m}), f_{k-1}(\mathbf{a}_{1:k-1})_{m+1:m+n(k-1)} \rangle
    \end{gather}
Sets $\mathcal{I, M, N}$ are called the \textbf{input, medium} and \textbf{output spaces} respectively and the function $g$ is called the \textbf{generator}.

Such a sequence can generate a class of boolean functions $\mathcal{C}:=(\mathscr{f}_k)_{k \in \mathbb{N}^*}$ where the set of variables are $\mathbf{Y}_{1:(d+n)k+m}$ and for all $k \in \mathbb{N}^*$,  $\mathbf{y} \in \mathscr{f}_k$ iff:
\begin{gather}
    \mathbf{y}_{1:dk}\in \mathcal{I}^k \subset \mathbb{B}^{d \times k} \\
    \mathbf{y}_{dk+1:(d+n)k+m} = f_k(\mathbf{y}_{1:dk})
\end{gather}
